Modeling Embedding Dimension Correlations via Convolutional Neural Collaborative Filtering

As the core of recommender system, collaborative filtering (CF) models the affinity between a user and an item from historical user-item interactions, such as clicks, purchases, and so on. Benefited from the strong representation power, neural networks have recently revolutionized the recommendation research, setting up a new standard for CF. However, existing neural recommender models do not explicitly consider the correlations among embedding dimensions, making them less effective in modeling the interaction function between users and items. In this work, we emphasize on modeling the correlations among embedding dimensions in neural networks to pursue higher effectiveness for CF. We propose a novel and general neural collaborative filtering framework, namely ConvNCF, which is featured with two designs: 1) applying outer product on user embedding and item embedding to explicitly model the pairwise correlations between embedding dimensions, and 2) employing convolutional neural network above the outer product to learn the high-order correlations among embedding dimensions. To justify our proposal, we present three instantiations of ConvNCF by using different inputs to represent a user and conduct experiments on two real-world datasets. Extensive results verify the utility of modeling embedding dimension correlations with ConvNCF, which outperforms several competitive CF methods.

==> nn3-preliminary.tex <==
\section{Preliminaries}
\label{sec:pre}
In this section, we demonstrate some technical background on neural CF models. We first introduce the task of CF on implicit feedback and the learning schema. We then simply exhibit general neural CF structure. 

%Before delving into the technical details, we generalize some basic notations. Throughout the paper, we use bold uppercase letter (e.g., $\textbf{P}$) to denote a matrix, bold lowercase letter to denote a vector (e.g., $\textbf{p}_u$), and calligraphic uppercase letter to denote a tensor (e.g., $\mathcal{S}$).
%Moreover, scalar $p_{u,k}$ denotes the $(u,k)$-th element of matrix $\textbf{P}$, and vector $\textbf{p}_u$ denotes the $u$-th row vector in $\textbf{P}$.
%Let $\mathcal{S}$ be 3D tensor, then scalar $s_{a,b,c}$ denotes the $(a,b,c)$-th element of tensor $\mathcal{S}$, and vector $\textbf{s}_{a,b}$ denotes the slice of $\mathcal{S}$ at the element $(a,b)$.


\subsection{Problem Formulation}
\label{subsec:cftask}

Recommender system aim to recommend interesting items to users. As a significant technique for recommender system, collaborative filtering~(CF) provides personalized recommending results to satisfy different user preferences, which are hardly collect in most cases but hidden in the user historical actions. Historical actions, such as the rating, purchasing or viewing of users on items, are easy to collect. From them, we can naturally imagine how to predict user preferences. For example, we can naturally assume that a user would like the items that his friends like, and a user would like the items similar to what he bought or visited. Analyzing related information and automatically making the estimations are the process of collaborating filtering.

CF models can be grouped into two types, memory-based CF and model-based CF. Memory-based CF models directly compute the similarity between users or items with the raw data. These implementations are clear but their disadvantages are obvious: when the observed user-item interactions are sparse~(the situation is very common in reality), judging the similarity from the raw data becomes difficult. Thus recent works focus on model-based CF, which predict the score of given user-item pair, and recommend the high scored pairs. Due to the popularity of model-based CF, all CF appeared in this paper refer to model-based CF models.

The data for CF are mostly treated as a matrix. Let $M$, $N$ indicate the number of users and the number of items respectively, the interactive information can be organized as a matrix $\textbf{Y}\in\mathbb{R}^{M\times N}$. The element $y_{ui}$ at the $u$-th row and $i$-th column indicates the observed interaction between user $u$ and item $i$. If $y_{ui}$ is able to refer to user preference, such as rating score, it is called explicit feedback. Otherwise, if $y_{ui}$ is just a record of user behaviours including clicking, browsing, purchasing, etc., it is called implicit feedback. In practice, it is very difficult to collect explicit feedback~(\eg ratings, comments). In contrast, implicit feedback, such as clicking, browsing, purchasing, etc., are recorded in a large amount in the log files. Therefore, implicit feedback is the mainstream data in recent CF tasks.

Since implicit feedback can only exhibit whether the user-item pair exists or not, the element $y_{ui}$ is defined as,
\begin{equation}
\label{eq:yui}
    y_{ui} = 
\begin{cases}
    1 & \text{if } (u,i) \text{ is observed,}\\
    0 & \text{otherwise.}
\end{cases}
\end{equation}

It is notable that, implicit feedback does not refer to the user preference strictly. For example, $y_{ui} = 1$ indicates that user $u$ has an interaction with item $i$, but does not exactly mean that the user likes the item. Similarly, $y_{ui} = 0$ does not exactly mean that user $u$ dislikes item $i$. It may mean that user $u$ does not know item $i$, or even user $u$ likes item $i$. The way treating these observations is crucial. We will seriously discuss that in Section~\ref{subsec:training}.



\subsection{Neural Collaborative Filtering}
\label{subsec:ncf}
% collaborative filterin focus on representation learning and predictive function. The key problem on predictive function is the absence of feature dimensions correlations. 


% this may should be in section NCF
The key to build a CF model lies in twofold: 1) how to represent a user and an item, and 2) how to build the predictive function based on user and item representations.
In most cases, the users and items are represented as embeddings. Since there are many classic embedding designs~\cite{he2016vbpr,kabbur2013fism,koren2008factorization}, here we do not discuss the design of embedding but explore the predictive function. We just let $f^U(u)$ indicate user $u$ and $f^I(i)$ indicate item $i$, where $f^U(\cdot)$ and $f^I(\cdot)$ indicate the function converting ids to embeddings. With the predefined embeddings, we explore how to better build the predictive function $\mathcal{Y}(u,i)$.

Neural collaborative filtering~(NCF) is a kind of neural network designed predictive function. By leveraging powerful neural network, NCF obtains the state-of-the-art performance. Referring to the definitions in the neural network, we call the operations in NCF as a layer, and organize them as a pipeline. Through the pipeline, data is transmitted from lower layer to higher layer. Formally, the network structure is defined in Equation~\ref{eq:nn}.


\begin{equation}
    \label{eq:nn}
    \begin{aligned}
        \phi_0 &= \mathcal{F}(f^U(u),f^I(i))\\
        \phi_l &= a_l(\mathcal{L}_l(\phi_{l-1}))\\
        \hat{y}_{ui} &= \phi_L\\
    \end{aligned}
\end{equation}


where $\mathcal{F}(\cdot)$ is a function combining user embedding and item embedding, $\mathcal{L}_*$ indicate the core function of the layers, $a_*$ indicate the activation functions such as ReLU~\cite{nair2010rectified}, and $\phi_*$ are vectors indicating the output of the layers. The prediction $\hat{y}_{ui}$ is the output of $L$-th layer. It is notable that the type and property of neural network are determined by the implementation of $\mathcal{L}_*$, which we will discuss in Section~\ref{subsubsec:conv_mlp}.

Multi-Layer Perceptron~(MLP) indicates that all the layers are fully-connected layers. Convolutional 

To apply the user and item information to neural network, it is required to combine the user embedding and item embedding with $\mathcal{F}(\cdot)$, as the $\phi_0$ in Equation~\ref{eq:nn}. The recent two major definitions of $\mathcal{F}(\cdot)$ are element-wise product and concatenation. 

\textbf{Element-wise Product} generates the combined vector by multiplying the corresponding dimension of user embedding and item embedding, which is formally defined in Equation~\ref{eq:ewp}

\begin{equation}
\label{eq:ewp}
\mathcal{F}(f^U(u),f^I(i)) = 
\left(
\begin{matrix}
    f^U(u)_1\cdot f^I(i)_1,\\
    f^U(u)_2\cdot f^I(i)_2,\\
    \cdots, \\
    f^U(u)_K\cdot f^I(i)_K\\
\end{matrix}
\right)
\end{equation}

It stems from vector similarity. If summing the elements in the result vector, it is actually the inner product which is always used to compute the similarity between two vectors. Thus element-wise product is considered to be an effective method and widely used in classic CF models~\cite{koren2009matrix,kabbur2013fism,koren2008factorization}. Some NCFs, such as JRL~\cite{zhang2017joint}, and GMF~\cite{he2017neural} take it for embedding combination. However, after element-wise product, the raw information is lost.

\textbf{Concatenation} means the two embeddings are concatenated, as shown in Equation~\ref{eq:cc}. It keeps the raw information and expects the neural network to learn the potential relations. However, due to the strong expressiveness of NN models and the insufficiency of data, learning the rules from such data are always difficult. It is observed that the MLP~\cite{gardner1998artificial} CF model performs a bit worse than JRL~\cite{zhang2017joint}.

\begin{equation}
\label{eq:cc}
\mathcal{F}(f^U(u),f^I(i)) = 
\left(
\begin{matrix}
    f^U(u)\\
    f^I(i)
\end{matrix}
\right)
\end{equation}

\textbf{The drawback} of these combining functions is that they assume  the  embedding  dimensions  are  independent  of  each other, that is, no correlations among the dimensions are captured. Arguably, the following MLP network can approximate any continuous function~\cite{cybenko1989approximation}, therefore it might be capable of capturing  the  possible  correlations.  However,  such  process is rather implicit and as such, it may be ineffective in capturing certain  relations -- an  evidence  is  from~\cite{tay2018latent} showing  that much more parameters have to be used in order to approximate the simple multiplicative relation.




